Equivariant Perturbation in Gomory and Johnson's Infinite Group Problem. IV. The General Unimodular Two-Dimensional Case

We study an abstract setting for cutting planes for integer programming called the infinite group problem. In this abstraction, cutting planes are computed via cut generating function that act on the simplex tableau. In this function space, cut generating functions are classified as minimal, extreme, and facets as a proxy for understanding the strength or potential importance of these functions. Prior work developed algorithms for testing minimality, extremality, and facetness for cut generating functions applied to 1-row tableau and to some 2-row tableau in a restricted setting. We complement and generalize this work by giving an algorithm for testing the extremality of a large class of minimal valid functions for the two-dimensional infinite group problem. Along the way, we develop results of independent interest on functional equations and infinite systems of linear equations.

==> function-poset.tex <==



